Overcoming Algorithm Aversion: A Comparison between Process and Outcome Control

Algorithm aversion occurs when humans are reluctant to use algorithms despite their superior performance. Studies show that giving users outcome control by providing agency over how models' predictions are incorporated into decision-making mitigates algorithm aversion. We study whether algorithm aversion is mitigated by process control, wherein users can decide what input factors and algorithms to use in model training. We conduct a replication study of outcome control, and test novel process control study conditions on Amazon Mechanical Turk (MTurk) and Prolific. Our results partly confirm prior findings on the mitigating effects of outcome control, while also forefronting reproducibility challenges. We find that process control in the form of choosing the training algorithm mitigates algorithm aversion, but changing inputs does not. Furthermore, giving users both outcome and process control does not reduce algorithm aversion more than outcome or process control alone. This study contributes to design considerations around mitigating algorithm aversion.

==> tables/demographics_all.tex <==
\begin{table}[h]\centering\small
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption{Demographics of Participants from MTurk, Prolific and Both (Pooled)}
\begin{tabular}{p{5cm}p{0.6cm}p{0.6cm}p{0.6cm}}
& Mturk & Prolific & Pooled \\
\hline\hline
\% Female                                                               & 40.8  & 65.7     & 51.9   \\ [0.02cm]
\% Male                                                                & 56.8  & 28.0     & 43.9   \\ [0.02cm]
\% White                                                                 & 84.1  & 74.4     & 79.7   \\ [0.02cm]
\% Black or African American                                             & 8.0   & 6.9      & 7.5    \\ [0.02cm]
\% Hispanic or Latino                                                    & 11.2  & 10.8     & 11.1   \\ [0.02cm]
Average Age (Year)                                                           & 38.5  & 34.6     & 36.8   \\ [0.02cm]
\% Some college and above                                                & 92.1  & 87.0     & 89.8   \\ [0.02cm]
\% High school/GED                                                       & 7.4   & 11.4     & 9.2    \\ [0.02cm]
Average Confidence in Math            & 3.3  & 2.6     & 3.0   \\ [0.02cm]
\% Participated in Algorithm-related Studies Previously & 78.2  & 51       & 66     \\ [0.02cm]
\hline
N   & 1,443  & 1,172     & 2,615 \\
\hline\hline
\multicolumn{4}{l}{\footnotesize Response categories where few respondents selected or declined to answer are dropped}\\
\multicolumn{4}{l}{\footnotesize Average confidence in math is converted from a survey question using a 5-point Likert scale}\\
\multicolumn{4}{l}{\footnotesize where 1 is "not confident", 5 is "extremely confident"}\\
\end{tabular}
\label{table:demographics_all}
\end{table}

==> tables/likelihood_filtered.tex <==
\begin{table}[htbp]\centering
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption{Intervention Effects on Likelihood of Choosing the Model}
\begin{tabular}{l*{6}{c}}
\hline\hline
            &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}&\multicolumn{1}{c}{(6)}\\
            &\multicolumn{1}{c}{MTurk}&\multicolumn{1}{c}{MTurk}&\multicolumn{1}{c}{Prolific}&\multicolumn{1}{c}{Prolific }&\multicolumn{1}{c}{Pooled}&\multicolumn{1}{c}{Pooled }\\
\hline
stated model error&       0.021         &       0.014         &      -0.023         &      -0.026         &      -0.009         &      -0.008         \\
            &     (0.021)         &     (0.022)         &     (0.019)         &     (0.020)         &     (0.014)         &     (0.014)         \\
[1em]
change outcome by 10&       0.237\sym{***}&       0.234\sym{***}&                     &                     &       0.253\sym{***}&       0.243\sym{***}\\
            &     (0.059)         &     (0.060)         &                     &                     &     (0.050)         &     (0.051)         \\
[1em]
change outcome freely&       0.164\sym{**} &       0.183\sym{**} &      -0.040         &      -0.031         &       0.041         &       0.044         \\
            &     (0.057)         &     (0.057)         &     (0.058)         &     (0.058)         &     (0.041)         &     (0.041)         \\
[1em]
change input&      -0.038         &      -0.015         &       0.041         &       0.048         &       0.005         &       0.002         \\
            &     (0.085)         &     (0.087)         &     (0.079)         &     (0.080)         &     (0.057)         &     (0.057)         \\
[1em]
change algorithm  &       0.227\sym{**} &       0.238\sym{***}&       0.152\sym{*}  &       0.146         &       0.185\sym{***}&       0.188\sym{***}\\
            &     (0.071)         &     (0.070)         &     (0.076)         &     (0.075)         &     (0.052)         &     (0.052)         \\
[1em]
change outcome and input&       0.069         &       0.028         &       0.209\sym{*}  &       0.200\sym{*}  &       0.159\sym{*}  &       0.163\sym{**} \\
            &     (0.092)         &     (0.094)         &     (0.084)         &     (0.085)         &     (0.062)         &     (0.062)         \\
[1em]
change outcome and algorithm&      -0.158         &      -0.179\sym{*}  &       0.068         &       0.069         &      -0.026         &      -0.030         \\
            &     (0.084)         &     (0.083)         &     (0.086)         &     (0.085)         &     (0.061)         &     (0.060)         \\
[1em]
demographics &               &     \cmark  &               &     \cmark         &              &      \cmark        \\
\hline
\(N\)       &         960         &         960         &        1078         &        1078         &        2038         &        2038         \\
\(R^{2}\)   &       0.040         &       0.075         &       0.038         &       0.069         &       0.035         &       0.049         \\
adj. \(R^{2}\)&       0.033         &       0.045         &       0.033         &       0.042         &       0.031         &       0.035         \\
\hline\hline
\multicolumn{7}{l}{\footnotesize Prolific specification excludes change outcome by 10 because this condition was not}\\
\multicolumn{7}{l}{\footnotesize The sample includes participants who passed attention checks and who are from adjust-by-10 (proposed bonus scheme)}\\
\multicolumn{7}{l}{\footnotesize Standard errors in parentheses}\\
\multicolumn{7}{l}{\footnotesize \sym{*} \(p<0.05\), \sym{**} \(p<0.01\), \sym{***} \(p<0.001\)}\\
\end{tabular}
\label{table:outcome_likelihood_of_choosing_model} 
\end{table}


==> tables/outcome_aae.tex <==
\begin{table}[h]\centering\small
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption{Intervention Effects on Average Absolute Error}
\begin{tabular}{l*{3}{c}}
\hline\hline
            &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}\\
            &\multicolumn{1}{c}{MTurk}&\multicolumn{1}{c}{Prolific}&\multicolumn{1}{c}{Pooled}\\
\hline
stated model error&      -0.083         &      -0.327         &      -0.189         \\
            &     (0.221)         &     (0.230)         &     (0.159)         \\
[1em]
observed model error&       0.727\sym{***}&       0.678\sym{***}&       0.706\sym{***}\\
            &     (0.046)         &     (0.054)         &     (0.035)         \\
[1em]
change outcome by 10&      -1.601\sym{*}  &               &      -1.927\sym{***}\\
            &     (0.623)         &                  &     (0.555)         \\
[1em]
change outcome freely&      -0.396         &       0.119         &      -0.125         \\
            &     (0.576)         &     (0.724)         &     (0.450)         \\
[1em]
change input&       0.871         &       0.590         &       0.758         \\
            &     (0.881)         &     (1.026)         &     (0.664)         \\
[1em]
change algorithm  &      -2.112\sym{***}&      -2.255\sym{**} &      -2.161\sym{***}\\
            &     (0.637)         &     (0.854)         &     (0.515)         \\
[1em]
change outcome and input&      -0.007         &       0.596         &       0.302         \\
            &     (0.921)         &     (1.034)         &     (0.684)         \\
[1em]
change outcome and algorithm&       2.641\sym{***}&       1.652         &       2.169\sym{***}\\
            &     (0.796)         &     (0.943)         &     (0.604)         \\
[1em]
\_cons      &      11.320\sym{**} &      17.886\sym{***}&      14.132\sym{***}\\
            &     (4.320)         &     (4.448)         &     (3.081)         \\
\hline
\(N\)       &        1443         &        1172         &        2615         \\
\hline\hline
\multicolumn{4}{l}{\footnotesize Standard errors in parentheses}\\
\multicolumn{4}{l}{\footnotesize \sym{*} \(p<0.05\), \sym{**} \(p<0.01\), \sym{***} \(p<0.001\)}\\
\end{tabular}
\label{table:outcome_aae}
\end{table}


==> tables/outcome_deviation.tex <==
\begin{table}[htbp]\centering\small
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption{Intervention Effects on Average Absolute Deviation}
\begin{tabular}{l*{3}{c}}
\hline\hline
            &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}\\
            &\multicolumn{1}{c}{MTurk}&\multicolumn{1}{c}{Prolific}&\multicolumn{1}{c}{Pooled}\\
\hline
stated model error&       0.041         &      -0.115         &       0.039         \\
            &     (0.396)         &     (0.406)         &     (0.283)         \\
[1em]
observed model error&       0.001         &       0.040         &       0.024         \\
            &     (0.083)         &     (0.097)         &     (0.064)         \\
[1em]
change outcome by 10&      -1.530         &              &      -2.258\sym{*}  \\
            &     (1.169)         &                  &     (1.014)         \\
[1em]
change outcome freely&       1.194         &       3.388\sym{*}  &       2.282\sym{**} \\
            &     (1.074)         &     (1.333)         &     (0.839)         \\
[1em]
change input&       0.247         &       0.536         &       0.425         \\
            &     (1.720)         &     (1.955)         &     (1.288)         \\
[1em]
change algorithm  &      -4.980\sym{***}&      -4.884\sym{**} &      -4.894\sym{***}\\
            &     (1.309)         &     (1.700)         &     (1.047)         \\
[1em]
change outcome and input&       1.897         &      -0.382         &       0.785         \\
            &     (1.787)         &     (1.970)         &     (1.320)         \\
[1em]
change outcome and algorithm&       5.196\sym{***}&       2.654         &       4.037\sym{***}\\
            &     (1.508)         &     (1.832)         &     (1.168)         \\
[1em]
\_cons      &       9.222         &      13.310         &       9.554         \\
            &     (7.734)         &     (7.812)         &     (5.495)         \\
\hline
\(N\)       &        1,443         &        1,172         &        2,615         \\
\hline\hline
\multicolumn{4}{l}{\footnotesize Standard errors in parentheses}\\
\multicolumn{4}{l}{\footnotesize \sym{*} \(p<0.05\), \sym{**} \(p<0.01\), \sym{***} \(p<0.001\)}\\
\end{tabular}
\end{table}


==> tables/outcome_likelihood_of_choosing_model.tex <==
\begin{table}[h]\centering\small
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption{Intervention Effects on Likelihood of Choosing the Model}
\begin{tabular}{l*{3}{c}}
\hline\hline
            &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}\\
            &\multicolumn{1}{c}{MTurk}&\multicolumn{1}{c}{Prolific}&\multicolumn{1}{c}{Pooled}\\
\hline
stated model error &       0.014         &      -0.028         &      -0.008         \\
            &     (0.017)         &     (0.019)         &     (0.013)         \\
[1em]
change outcome by 10 &       0.213\sym{***}&                     &       0.237\sym{***}\\
            &     (0.051)         &                     &     (0.044)         \\
[1em]
change outcome freely &       0.149\sym{**} &      -0.026         &       0.053         \\
            &     (0.048)         &     (0.055)         &     (0.036)         \\
[1em]
change input&      -0.016         &       0.052         &       0.012         \\
            &     (0.069)         &     (0.077)         &     (0.051)         \\
[1em]
change algorithm &       0.169\sym{**} &       0.188\sym{**} &       0.173\sym{***}\\
            &     (0.060)         &     (0.071)         &     (0.046)         \\
[1em]
change outcome and input&       0.011         &       0.193\sym{*}  &       0.113\sym{*}  \\
            &     (0.075)         &     (0.082)         &     (0.055)         \\
[1em]
change outcome and algorithm&      -0.125         &       0.028         &      -0.042         \\
            &     (0.070)         &     (0.080)         &     (0.053)         \\
[1em]
\_cons      &       0.268         &       1.035\sym{**} &       0.688\sym{**} \\
            &     (0.337)         &     (0.372)         &     (0.250)         \\
\hline
\(N\)       &        1,369         &        1,172         &        2,541         \\
\hline\hline
\multicolumn{4}{l}{\footnotesize Standard errors in parentheses}\\
\multicolumn{4}{l}{\footnotesize Prolific specification excludes change outcome by 10 because this condition was not}\\
\multicolumn{4}{l}{\footnotesize replicated on Prolific}\\
\multicolumn{4}{l}{\footnotesize \sym{*} \(p<0.05\), \sym{**} \(p<0.01\), \sym{***} \(p<0.001\)}\\
\end{tabular}
\label{table:outcome_likelihood_of_choosing_model}
\end{table}


